Rethinking the Evaluation of Microservice RCA with a Fault Propagation-Aware Benchmark

While cloud-native microservice architectures have revolutionized software development, their inherent operational complexity makes failure Root Cause Analysis (RCA) a critical yet challenging task. Numerous data-driven RCA models have been proposed to address this challenge. However, we find that the benchmarks used to evaluate these models are often too simple to reflect real-world scenarios. Our preliminary study reveals that simple rule-based methods can achieve performance comparable to or even surpassing state-of-the-art (SOTA) models on four widely used public benchmarks. This finding suggests that the oversimplification of existing benchmarks might lead to an overestimation of the performance of RCA methods. To further investigate the oversimplification issue, we conduct a systematic analysis of popular public RCA benchmarks, identifying key limitations in their fault injection strategies, call graph structures, and telemetry signal patterns. Based on these insights, we propose an automated framework for generating more challenging and comprehensive benchmarks that include complex fault propagation scenarios. Our new dataset contains 1,430 validated failure cases from 9,152 fault injections, covering 25 fault types across 6 categories, dynamic workloads, and hierarchical ground-truth labels that map failures from services down to code-level causes. Crucially, to ensure the failure cases are relevant to IT operations, each case is validated to have a discernible impact on user-facing SLIs. Our re-evaluation of 11 SOTA models on this new benchmark shows that they achieve low Top@1 accuracies, averaging 0.21, with the best-performing model reaching merely 0.37, and execution times escalating from seconds to hours.

==> algorithms/detector.tex <==
\begin{algorithm}[t]
\footnotesize
\caption{User-aware Anomaly Detection Logic}
\label{alg:detector}
\begin{algorithmic}[1]
\Function{DetectAnomaly}{$curr, hist, cfg$}
    \If{count($hist.latency$) < 5} \Return \texttt{NO ANOMALY} \EndIf
    \State $mean\_hist \leftarrow \text{mean}(hist.latency)$; $p99\_hist \leftarrow \text{percentile}(hist.latency, 99)$
    \If{$cfg.filter\_baseline$ \textbf{and} ($mean\_hist > cfg.base\_avg$ \textbf{or} $p99\_hist > cfg.base\_p99$)} \Return \texttt{NO ANOMALY} \EndIf
    \State $has\_latency\_anomaly \leftarrow \Call{CheckLatencyAnomaly}{curr.latency, mean\_hist, cfg}$
    \State $has\_rate\_anomaly \leftarrow \Call{CheckRateAnomaly}{curr.rate, hist.rate}$
    \If{$has\_latency\_anomaly$ \textbf{and} $has\_rate\_anomaly$} \Return \texttt{HAS ANOMALY} \EndIf
    \If{$has\_rate\_anomaly$ \textbf{or} $has\_latency\_anomaly$} \Return \texttt{HAS ANOMALY} \EndIf
    \State \Return \texttt{NO ANOMALY}
\EndFunction

\Function{CheckLatencyAnomaly}{$curr\_latency, mean\_hist, cfg$}
    \If{$curr\_latency \leq mean\_hist$ \textbf{or} $curr\_latency > cfg.hard\_thresh$} \Return $curr\_latency > cfg.hard\_thresh$ \EndIf
    \State $threshold \leftarrow (mean\_hist < cfg.small\_base\_thresh) ? cfg.abs\_thresh : mean\_hist \times \Call{GetMultiplier}{mean\_hist, cfg}$
    \State \Return $curr\_latency > threshold$
\EndFunction

\Function{CheckRateAnomaly}{$curr\_rate, hist\_rate$}
    \State \Return $\Call{Z\_Test}{curr\_rate, hist\_rate} < 0.05$ \textbf{and} $(\text{mean}(hist\_rate) - curr\_rate) > 0.03$
\EndFunction
\end{algorithmic}
\end{algorithm}

==> figures/rq5_case_study_signal_loss.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{\textwidth}
\centering
    \includegraphics[width=\textwidth]{figures/rq5_case_study_signal_loss_figure.pdf}
    \caption{Case Study: Signal-Loss Blind Spots. When faults occurred in Seat Service, the requests are missing in the downstream applications.}
    \label{fig:rq5_case_study_signal_loss}
  \end{minipage}
  \hfill
  \begin{minipage}{0.43\textwidth}
    \centering
    \tiny
    \begin{tcolorbox}[
      colback=gray!5,
      colframe=gray!50,
      boxrule=0.5pt,
      left=2mm,
      right=2mm,
      top=2mm,
      bottom=2mm
    ]
    \begin{verbatim}
 1  // A common anti-pattern causing a semantic gap.
 2  for (item in batch_items) {
 3      try {
 4          sender.send(item);
 5      } catch (Exception e) {
 6          // The error is logged...
 7          LOGGER.error("Failed to send item: {}", item);
 8          // ...but the exception is suppressed.
 9      }
10  }
11  // The function reports success to the caller,
12  // regardless of any errors that occurred inside the loop.
13  return new Response(SUCCESS_CODE, "Batch processed.", null);
    \end{verbatim}
    \end{tcolorbox}
    
    \caption{An example of flawed application logic where internal errors are logged but masked by a successful return status, creating a semantic gap between logs and high-level metrics/traces.}
    \label{lst:semantic-gap}
  \end{minipage}
\end{figure}
